An Information-Theoretic View of Mixed-Delay Traffic in 5G and 6G

Fifth generation mobile communication systems (5G) have to accommodate both Ultra-Reliable Low-Latency Communication (URLLC) and enhanced Mobile Broadband (eMBB) services. While, eMBB applications support high data rates, URLLC services aim at guaranteeing low-latencies and high-reliabilities. eMBB and URLLC services are scheduled on the same frequency band, where the different latency requirements of the communications render the coexistence challenging. In this survey, we review, from an information theoretic perspective, coding schemes that simultaneously accommodate URLLC and eMBB transmissions and show that they outperform traditional scheduling approaches. Various communication scenarios are considered, including point-to-point channels, broadcast channels, interference networks, cellular models, and cloud radio access networks (C-RANs). The main focus is on the set of rate pairs that can simultaneously be achieved for URLLC and eMBB messages, which well captures the tension between the two types of communications. We also discuss finite-blocklength results where the measure of interest is the set of error probability pairs that can simultaneously be achieved on the two communication regimes.

==> figure-CRAN.tex <==
%\usepackage{graphicx}
%\usepackage{amsmath,amssymb,dsfont,bbm,epstopdf,pgfplots,mathtools,enumitem,mathrsfs, bbm, algpseudocode , graphicx, tikzpeople} 
%\usepackage[normalem]{ulem}
%\usepackage{color}
%\usepackage{cite}%hyperref}
%\usepackage{graphics}
%\usepackage{tikz}
%\usepackage{pgfplots}
%\usepackage{subcaption}
%\usetikzlibrary{shapes, arrows, decorations.markings, arrows.meta}
%\usetikzlibrary{patterns} % LATEX and plain TEX when using Tik Z
%\allowdisplaybreaks
%\graphicspath{{.}{./Figures/}} % path to figures
%\allowdisplaybreaks[4] % Allows the align environment to wrap over pages.
%\input{def.tex}
%\usetikzlibrary{decorations.pathreplacing,decorations.markings,shapes.geometric}
%\usetikzlibrary{shapes, arrows, decorations.markings, arrows.meta, tikzmark,fit}
%\usetikzlibrary{backgrounds,calc,shadings,shapes.arrows,shapes.symbols,shadows}
%\usetikzlibrary{positioning}
%\usepackage{tikz-3dplot}
%\usepackage{graphicx}
%\usepackage{amsmath,amssymb,dsfont,bbm,epstopdf,pgfplots} 
%\usepackage{color}
%\usepackage{cite}%hyperref}
%\usepackage{graphics}
%\usepackage{tikz}
%\usepackage{pgfplots}
%\usetikzlibrary{shapes, arrows, decorations.markings, arrows.meta, tikzmark,fit,backgrounds}
%\usepackage{ellipsis}
%\usetikzlibrary{calc}
%\usetikzlibrary{decorations.pathreplacing,decorations.markings,shapes.geometric}
%\usepackage{graphicx} % Allows including images
%\usepackage{booktabs} % Allows the use of \toprule, \midrule and \bottomrule in tables
%\usetikzlibrary{patterns} % LATEX and plain TEX when using Tik Z
%\allowdisplaybreaks
%\graphicspath{{.}{./Figures/}} % path to figures
%\usepackage{graphicx}
%\usepackage{amsmath,amssymb,dsfont,bbm,epstopdf,pgfplots, niceframe, fonttable} 
%\usepackage{color}
%\usepackage{cite}%hyperref}
%\usepackage{graphics}
%\usepackage{tikz}
%\usepackage{pgfplots,wasysym, marvosym}
%%\DeclareFontFamily{U}{umranda}{}
%%\DeclareFontShape{U}{umranda}{m}{n}{<-> umranda}{52}
%%\DeclareFontFamily{U}{umranda}{52}
%\usetikzlibrary{shapes, arrows, decorations.markings, arrows.meta}
%\usetikzlibrary{patterns} % LATEX and plain TEX when using Tik Z
%\allowdisplaybreaks
%\graphicspath{{.}{./Figures/}} % path to figures
%\allowdisplaybreaks[4] 
%\usepackage{relsize}
%\allowdisplaybreaks[4] 
%\usepackage{relsize}
%\tikzset{arr/.style={line width=2.5pt, {-Latex[left]}, #1}}
%\tikzset{arrr/.style={line width=2.5pt, {-Latex[right]}, #1}}
%\newcommand{\bigqm}[1][1]{\text{\larger[#1]{\textbf{?}}}}
% \renewcommand{\familydefault}{\rmdefault}
%
%
%\usepackage{graphicx} % Allows including images
%\usepackage{booktabs} % Allows the use of \toprule, \midrule and \bottomrule in tables
%\usetikzlibrary{fit}
%\tikzset{
%  comp/.style = {
%    minimum width  = 8cm,
%    minimum height = 4.5cm,
%    text width     = 8cm,
%    inner sep      = 0pt,
%    text           = green,
%    align          = center,
%    font           = \Huge,
%    transform shape,
%    thick
%  },
%  Monitor/.style = {draw = none, xscale = 18/16, yscale = 11/9},
%  display/.style = {shading = axis, left color = black!60, right color = black},
%  ut/.style      = {fill = gray}
%}
%\tikzset{
%  computer/.pic = {
%    % screen (with border)
%    \node(-m) [comp, pic actions, Monitor]
%      {\phantom{\parbox{\linewidth}{\tikzpictext}}};
%    % display (without border)
%    \node[comp, pic actions, display] {\tikzpictext};
%    \begin{scope}[x = (-m.east), y = (-m.north)]
%      % filling the lower part
%      \path[pic actions, draw = none]
%        ([yshift=2\pgflinewidth]-0.1,-1) -- (-0.1,-1.3) -- (-1,-1.3) --
%        (-1,-2.4) -- (1,-2.4) -- (1,-1.3) -- (0.1,-1.3) --
%        ([yshift=2\pgflinewidth]0.1,-1);
%      % filling the border of the lower part
%      \path[ut]
%        (-1,-2.4) rectangle (1,-1.3)
%        (-0.9,-1.4) -- (-0.7,-2.3) -- (0.7,-2.3) -- (0.9,-1.4) -- cycle;
%      % drawing the frame of the whole computer
%      \path[pic actions, fill = none]
%        (-1,1) -- (-1,-1) -- (-0.1,-1) -- (-0.1,-1.3) -- (-1,-1.3) --
%        (-1,-2.4) coordinate(sw)coordinate[pos=0.5] (-b west) --
%        (1,-2.4) -- (1,-1.3) coordinate[pos=0.5] (-b east) --
%        (0.1,-1.3) -- (0.1,-1) -- (1,-1) -- (1,1) -- cycle;
%      % node around the whole computer
%      \node(-c) [fit = (sw)(-m.north east), inner sep = 0pt] {};
%    \end{scope}
%  }
%}
%%\pgfkeys{/pgf/.cd,
%%  parallelepiped offset x/.initial=2mm,
%%  parallelepiped offset y/.initial=2mm
%%}
%%\pgfdeclareshape{parallelepiped}
%\makeatletter
%\pgfkeys{/pgf/.cd,
%  parallelepiped offset x/.initial=2mm,
%  parallelepiped offset y/.initial=2mm
%}
%\pgfdeclareshape{parallelepiped}
%{
%  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
%  \inheritanchorborder[from=rectangle]
%  \inheritanchor[from=rectangle]{north}
%  \inheritanchor[from=rectangle]{north west}
%  \inheritanchor[from=rectangle]{north east}
%  \inheritanchor[from=rectangle]{center}
%  \inheritanchor[from=rectangle]{west}
%  \inheritanchor[from=rectangle]{east}
%  \inheritanchor[from=rectangle]{mid}
%  \inheritanchor[from=rectangle]{mid west}
%  \inheritanchor[from=rectangle]{mid east}
%  \inheritanchor[from=rectangle]{base}
%  \inheritanchor[from=rectangle]{base west}
%  \inheritanchor[from=rectangle]{base east}
%  \inheritanchor[from=rectangle]{south}
%  \inheritanchor[from=rectangle]{south west}
%  \inheritanchor[from=rectangle]{south east}
%  \backgroundpath{
%    % store lower right in xa/ya and upper right in xb/yb
%    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
%    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
%    \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/parallelepiped
%      offset x}}
%    \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/parallelepiped
%      offset y}}
%    \def\ppd@offset{\pgfpoint{\pgfutil@tempdima}{\pgfutil@tempdimb}}
%    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
%    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
%    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
%    \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
%    \pgfpathclose
%    \pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
%    \pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@ya}}{\ppd@offset}}
%    \pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@yb}}{\ppd@offset}}
%    \pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xa}{\pgf@yb}}{\ppd@offset}}
%    \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
%    \pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
%    \pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@yb}}{\ppd@offset}}
%  }
%}
%\makeatother
%
%\tikzset{
%  ports/.style={
%    line width=0.3pt,
%    top color=gray!20,
%    bottom color=gray!80
%  },
%  server/.style={
%    parallelepiped,
%    fill=white, draw,
%    minimum width=0.35cm,
%    minimum height=0.75cm,
%    parallelepiped offset x=3mm,
%    parallelepiped offset y=2mm,
%    xscale=-1,
%    path picture={
%      \draw[top color=gray!5,bottom color=gray!40]
%      (path picture bounding box.south west) rectangle 
%      (path picture bounding box.north east);
%      \coordinate (A-center) at ($(path picture bounding box.center)!0!(path
%        picture bounding box.south)$);
%      \coordinate (A-west) at ([xshift=-0.575cm]path picture bounding box.west);
%      \draw[ports]([yshift=0.1cm]$(A-west)!0!(A-center)$)
%        rectangle +(0.2,0.065);
%      \draw[ports]([yshift=0.01cm]$(A-west)!0.085!(A-center)$)
%        rectangle +(0.15,0.05);
%      \fill[black]([yshift=-0.35cm]$(A-west)!-0.1!(A-center)$)
%        rectangle +(0.235,0.0175);
%      \fill[black]([yshift=-0.385cm]$(A-west)!-0.1!(A-center)$)
%        rectangle +(0.235,0.0175);
%      \fill[black]([yshift=-0.42cm]$(A-west)!-0.1!(A-center)$)
%        rectangle +(0.235,0.0175);
%    }  
%  },
%}
%\begin{document}
%\begin{center}
%\footnotesize
% \begin{tabular}{ l | c | c | l}
%    \hline
%    Model & Delay Type & Applications & Section\\ \hline
%    P2P & & & \shortstack[l]{Sec~III.A: Rate pair  [34]-[36],  \\ Sec.~III.B: Error probability pair [24], [37]  }   \\ \hline
%    Broadcast channel &  & & Sec~IV: Rate pair [39]  \\ \hline
%%MAC & & & & \\ \hline
%Cooperative Networks & & & \shortstack[l]{Sec~V: DoF pair [41],[42],[43],[45] \\Error probability pair: Open problem}\\ \hline
%C-RAN &  & & \shortstack[l]{ Sec~VI: Rate pair [49]-[51], DoF pair [49] \\ Error probability pair: Open problem}\\ \hline
%  \end{tabular}
%\end{center}
\begin{figure}[t]
%\footnotesize
 \begin{subfigure}{0.6\textwidth}
%  \centering
 % \small
  %  \vspace*{-20pt}
 \begin{tikzpicture}[scale=1.1, >=stealth]
\centering
\tikzset{radiation/.style={{decorate,decoration={expanding waves,angle=0,segment length=4pt}}}}
%\node [draw=none] at (1.9,1.2) {Network};
\tikzstyle{myarrowss}=[line width=0.5mm,draw = red,fill=none,-triangle 45,postaction={draw, line width=0.8mm, shorten >=3mm, -}]
\tikzstyle{myarrowsss}=[line width=0.5mm,draw = blue,fill=none,-triangle 45,postaction={draw, line width=1mm, shorten >=3mm, -}]
\tikzstyle{myarrows}=[line width=0.9mm,draw = blue,fill=none,-triangle 45,postaction={draw, line width=3mm, shorten >=3mm, -}]
 \foreach \i in {-1.25,0,1.25} {
 \draw[very thick] (2.15+2*\i-2, 3) -- (2.15-2, 5);
\draw [thick, purple] (2+2*\i-2,2.4)--(2.15+2*\i-2, 3)--(2.3+2*\i-2,2.4);
\draw [thick, purple] (2.1+2*\i-2,2.8)--(2.3+2*\i-2,2.4)--(2+2*\i-2,2.4)--(2.2+2*\i-2,2.8);
\draw [fill = purple](2.15+2*\i-2,3.1) circle(0.1);
\draw[purple,radiation,decoration={angle=45}] (2.25+2*\i-2,3.1) -- +(10:0.5);
\draw[purple,radiation,decoration={angle=45}, rotate = 180] (2.25+2*\i-2-0.3,3.1-6.23) -- +(10:0.5);
}
\draw [fill = blue!10, rotate = 0](0,0) ellipse (4cm and 1.65cm); 
\node [draw=none] at (-2.55,4) {{{\textbf Fronthaul link}}};
\node[server, scale = 2.5] at (-0.5,6){};
\node[server, scale = 2.5] at (1.25,6){};
\node[cloud, cloud puffs=12.7, cloud ignores aspect, minimum width=4.5cm, minimum height=2cm, align=center, draw, fill= blue!50] (cloud) at (2.15-2, 5) {\textbf Cloud server};
\node[alice, female, mirrored, monitor, minimum size=0.75cm] at (2.5,-0.5){};
\node [draw=none] at (3,0.65) {{\Huge {\color{black}\Mobilefone}}};
\pic(comp0) [ draw, fill = orange!20 , scale = 0.1, yshift = -8cm] (0,0.75){computer};
\node[bob, mirrored, monitor, minimum size=0.75cm] at (0.9,1){};
\pic(comp0) [ draw, fill = orange , scale = 0.1, yshift = 10cm, xshift = -20cm] (0,0.75){computer};
\node [draw=none] at (-2.5,-0.75) {{\Huge {\color{black}\Mobilefone}}};
\draw (2.15-2*1.25-2, 2.4)-- (-1.8,1.1);
\draw (2.15-2*1.25-2, 2.4)-- (-2.8,-0.75);
\draw (2.15-2, 2.4)-- (-1.8+2.5,1.1);
\draw (2.15-2, 2.4)-- (-2.8+2.5,-0.55);
\draw (2.15+2*1.25-2, 2.4)-- (-1.8+5-0.3,1);
\draw (2.15+2*1.25-2, 2.4)-- (-2.8+5,-0.48);
\end{tikzpicture}
%\vspace*{-3ex}

  \caption{C-RAN}
  \label{fig1}
\end{subfigure}
 \begin{subfigure}{0.4\textwidth}
%  \centering
 % \small
  \vspace{2.1cm}
 \begin{tikzpicture}[scale=1.1, >=stealth]
\centering
\tikzset{radiation/.style={{decorate,decoration={expanding waves,angle=0,segment length=4pt}}}}
%\node [draw=none] at (1.9,1.2) {Network};
%\tikzstyle{myarrowss}=[line width=0.5mm,draw = red,fill=none,-triangle 45,postaction={draw, line width=0.8mm, shorten >=3mm, -}]
%\tikzstyle{myarrowsss}=[line width=0.5mm,draw = blue,fill=none,-triangle 45,postaction={draw, line width=1mm, shorten >=3mm, -}]
%\tikzstyle{myarrows}=[line width=0.9mm,draw = blue,fill=none,-triangle 45,postaction={draw, line width=3mm, shorten >=3mm, -}]
% \foreach \i in {-1.25,0,1.25} {
% \draw[very thick] (2.15+2*\i-2, 3) -- (2.15-2, 5);
%\draw [thick, purple] (2+2*\i-2,2.4)--(2.15+2*\i-2, 3)--(2.3+2*\i-2,2.4);
%\draw [thick, purple] (2.1+2*\i-2,2.8)--(2.3+2*\i-2,2.4)--(2+2*\i-2,2.4)--(2.2+2*\i-2,2.8);
%\draw [fill = purple](2.15+2*\i-2,3.1) circle(0.1);
%\draw[purple,radiation,decoration={angle=45}] (2.25+2*\i-2,3.1) -- +(10:0.5);
%\draw[purple,radiation,decoration={angle=45}, rotate = 180] (2.25+2*\i-2-0.3,3.1-6.23) -- +(10:0.5);
%}
%\draw [fill = blue!10, rotate = 0](0,0) ellipse (4cm and 1.65cm); 
%\node [draw=none] at (-2.55,4) {{{\textbf Fronthaul link}}};
%\node[server, scale = 2.5] at (-0.5,6){};
%\node[server, scale = 2.5] at (1.25,6){};
%\node[cloud, cloud puffs=12.7, cloud ignores aspect, minimum width=4.5cm, minimum height=2cm, align=center, draw, fill= blue!50] (cloud) at (2.15-2, 5) {\textbf Cloud server};
%\node[alice, female, mirrored, monitor, minimum size=0.75cm] at (2.5,-0.5){};
%\node [draw=none] at (3,0.65) {{\Huge {\color{black}\Mobilefone}}};
%\pic(comp0) [ draw, fill = orange!20 , scale = 0.1, yshift = -8cm] (0,0.75){computer};
%\node[bob, mirrored, monitor, minimum size=0.75cm] at (0.9,1){};
%\pic(comp0) [ draw, fill = orange , scale = 0.1, yshift = 10cm, xshift = -20cm] (0,0.75){computer};
%\node [draw=none] at (-2.5,-0.75) {{\Huge {\color{black}\Mobilefone}}};
%\draw (2.15-2*1.25-2, 2.4)-- (-1.8,1.1);
%\draw (2.15-2*1.25-2, 2.4)-- (-2.8,-0.75);
%\draw (2.15-2, 2.4)-- (-1.8+2.5,1.1);
%\draw (2.15-2, 2.4)-- (-2.8+2.5,-0.55);
%\draw (2.15+2*1.25-2, 2.4)-- (-1.8+5-0.3,1);
%\draw (2.15+2*1.25-2, 2.4)-- (-2.8+5,-0.48);
\node[regular polygon, regular polygon sides=6, draw, inner sep=1cm, fill = blue!10 ] at (0,0) {};
\node[regular polygon, regular polygon sides=6, draw, inner sep=1cm, fill = blue!10 ] at (2.2,-1.3) {};
\node[regular polygon, regular polygon sides=6, draw, inner sep=1cm, fill = blue!10] at (0,-2.59) {};
\node[regular polygon, regular polygon sides=6, draw, inner sep=1cm, fill = blue!10 ] at (2.2,-1.3-2.59) {};
 \foreach \i in {-0.2} 
  \foreach \j in {2.6, 5.2} {
\draw [thick, purple] (2+\i-2,2.4-\j)--(2.15+\i-2, 3- \j)--(2.3+\i-2,2.4- \j);
\draw [thick, purple] (2.1+\i-2,2.8- \j)--(2.3+\i-2,2.4 - \j)--(2+\i-2,2.4 - \j)--(2.2+\i-2,2.8 - \j);
\draw [fill = purple](2.15+\i-2,3.1 - \j) circle(0.1);
\draw[purple,radiation,decoration={angle=45}] (2.25+\i-2,3.1- \j) -- +(10:0.5);
%\draw[purple,radiation,decoration={angle=45}, rotate = 180] (2.25+2*\i-2-0.3,3.1-6.23 +\j) -- +(10:0.5);
}

\foreach \i in {2.1} 
  \foreach \j in {4, 6.6} {
\draw [thick, purple] (2+\i-2,2.4-\j)--(2.15+\i-2, 3- \j)--(2.3+\i-2,2.4- \j);
\draw [thick, purple] (2.1+\i-2,2.8- \j)--(2.3+\i-2,2.4 - \j)--(2+\i-2,2.4 - \j)--(2.2+\i-2,2.8 - \j);
\draw [fill = purple](2.15+\i-2,3.1 - \j) circle(0.1);
\draw[purple,radiation,decoration={angle=45}] (2.25+\i-2,3.1- \j) -- +(10:0.5);
%\draw[purple,radiation,decoration={angle=45}, rotate = 180] (2.25+2*\i-2-0.3,3.1-6.23 +\j) -- +(10:0.5);
}
\foreach \i in {0.6}
\foreach \j in {-0.6}{
\draw [fill = green](0+ \i,0+ \j) circle(0.1);
\draw [fill = green](0-0.1+ \i,-0.5-0.2+ \j) rectangle (0.2-0.1+ \i,0-0.2+ \j);
\draw [thick, black] (0+ \i,-0.1+ \j)--(0+ \i,-0.2+ \j);
}

\foreach \i in {1.5}
\foreach \j in {-1.9}{
\draw [fill = green](0+ \i,0+ \j) circle(0.1);
\draw [fill = green](0-0.1+ \i,-0.5-0.2+ \j) rectangle (0.2-0.1+ \i,0-0.2+ \j);
\draw [thick, black] (0+ \i,-0.1+ \j)--(0+ \i,-0.2+ \j);
}

\foreach \i in {0.75}
\foreach \j in {-3.2}{
\draw [fill = green](0+ \i,0+ \j) circle(0.1);
\draw [fill = green](0-0.1+ \i,-0.5-0.2+ \j) rectangle (0.2-0.1+ \i,0-0.2+ \j);
\draw [thick, black] (0+ \i,-0.1+ \j)--(0+ \i,-0.2+ \j);
}

\node [draw=none] at (-0.5,-0.6) {{\Large {\color{black}\Mobilefone}}};
\node [draw=none] at (-0.5,-0.5-3) {{ \Large {\color{black}\Mobilefone}}};
\node [draw=none] at (1.6,-4.8) {{ \Large {\color{black}\Mobilefone}}};
\node [draw=none] at (3,-2) {{ \Large {\color{black}\Mobilefone}}};
\node [draw=none] at (1.6,-0.5) {{ \Large {\color{black}\Mobilefone}}};
\draw [very thick , <->, blue] (0.6,-0.5)--(0.1,0.35);
\draw [very thick , <->, blue] (0.45,-0.9)--(0,0.35-2.3);
\draw [very thick , <->, blue] (0.7,-0.7)--(2.2,-0.95);
\draw [very thick , <->, blue] (2.2,-0.95)--(1.5,-1.8);
\draw [very thick , <->, blue] (1.4,-1.9)--(0.5,-2);
\draw [very thick , <->, blue] (2.2,-3.4)--(1.6,-2);
\draw [very thick , <->, blue] (2.1,-3.5)--(0.9,-3.2);
\draw [very thick , <->, blue] (0.7,-3.1)--(0.1,-2.3);
%
\draw [very thick , <->, red] (0.6,-3.2)--(-0.25,-3.3);
\draw [very thick , <->, red] (-0.5,-3.3)--(-0.1,-2.2);
\draw [very thick , <->, red] (1.6,-4.6)--(0.85,-3.2);
\draw [very thick , <->, red] (1.6,-4.6)--(2.1,-3.5);
\draw [very thick , <->, red] (1.9,-0.5)--(2.2,-0.8);
\draw [very thick , <->, red] (2.8,-2)--(1.6,-1.9);
\draw [very thick , <->, red] (2.8,-2)--(2.35,-1.1);
\draw [very thick , <->, red] (-0.3,-0.6)--(0.5,-0.65);
\draw [very thick , <->, red] (-0.55,-0.4)--(-0.2,0.4);


 \foreach \i in {4.2} 
  \foreach \j in {5.5} {
\draw [thick, purple] (2+\i-2,2.4-\j)--(2.15+\i-2, 3- \j)--(2.3+\i-2,2.4- \j);
\draw [thick, purple] (2.1+\i-2,2.8- \j)--(2.3+\i-2,2.4 - \j)--(2+\i-2,2.4 - \j)--(2.2+\i-2,2.8 - \j);
\draw [fill = purple](2.15+\i-2,3.1 - \j) circle(0.1);
\draw[purple,radiation,decoration={angle=45}] (2.25+\i-2,3.1- \j) -- +(10:0.5);
%\draw[purple,radiation,decoration={angle=45}, rotate = 180] (2.25+2*\i-2-0.3,3.1-6.23 +\j) -- +(10:0.5);
}
\node [draw=none] at (4.4,-4.8) {{\Large {\color{black}\Mobilefone}}};
\foreach \i in {4.4}
\foreach \j in {-3.5}{
\draw [fill = green](0+ \i,0+ \j) circle(0.1);
\draw [fill = green](0-0.1+ \i,-0.5-0.2+ \j) rectangle (0.2-0.1+ \i,0-0.2+ \j);
\draw [thick, black] (0+ \i,-0.1+ \j)--(0+ \i,-0.2+ \j);
}

\node [draw=none] at (5.4,-3) {{\footnotesize{Base station}}};
\node [draw=none] at (5.15,-4.1) {{\footnotesize{Relay}}};
\node [draw=none] at (5.2,-4.8) {{\footnotesize{Mobile}}};
\end{tikzpicture}
%\vspace*{-5ex}

  \caption{Cellular network with cooperation link}
  \label{fig1}
\end{subfigure}
 
 \caption{Infrastructures allowing to mitigate interference.}
\end{figure}~~%
